Space-filling groups

We introduce the notion of a space-filling group. These are finitely generated groups which admit an action on a compact space that carries a continuous cocycle which covers arbitrarily large portions of the space in a uniform manner. This notion is inspired by J. Kari's construction of a $\mathbb{Z}^2$-tileset that simulates Hilbert curves and its application to reversibility problems on cellular automata. We show that the property of being space-filling is always witnessed by a subshift, and consider computable, finitary and local variants. We show that the property of being space-filling is an invariant of quasi-isometry, and that the computable and finitary variants are also invariant under natural hypotheses. Furthermore, we provide interesting examples within the class of groups which are quasi-isometric to the hyperbolic space $\mathbb{H}^d$ for some $d\geq 1$ along with several stability properties of the class and applications to cellular automata and snake tiling problems on groups.

==> fig/hyperbolico.tex <==
\begin{tikzpicture}

	\begin{scope}[scale=0.3, shift={(0,0)}]
    \foreach \xx in {-12,0,12,24}{
	\begin{scope}[shift={(\xx,3)}, scale = 2]
	\draw (0,0) -- (0,3);
	\draw (0,3) to [controls=+(45:2) and +(135:2)] (6,3);
	\draw (6,3) -- (6,0);
	\draw (0,0) to [controls=+(45:1) and +(135:1)] (3,0);
	\draw (3,0) to [controls=+(45:1) and +(135:1)] (6,0);
	\end{scope}
	}
	\foreach \xx in {-12,-6,...,30}{
	\begin{scope}[shift={(\xx,0)}]
	\draw (0,0) -- (0,3);
	\draw (0,3) to [controls=+(45:2) and +(135:2)] (6,3);
	\draw (6,3) -- (6,0);
	\draw (0,0) to [controls=+(45:1) and +(135:1)] (3,0);
	\draw (3,0) to [controls=+(45:1) and +(135:1)] (6,0);
	\end{scope}
	}
	\foreach \xx in {-12,-9,...,33}{
	\begin{scope}[shift={(\xx,-3)},scale=0.5]
	\draw (0,0) -- (0,6);
	\draw (0,6) to [controls=+(45:2) and +(135:2)] (6,6);
	\draw (6,6) -- (6,0);
	\draw (0,0) to [controls=+(45:1) and +(135:1)] (3,0);
	\draw (3,0) to [controls=+(45:1) and +(135:1)] (6,0);
	\end{scope}
	}
	\foreach \xx in {-12,-10.5,...,34.5}{
	\begin{scope}[shift={(\xx,-6)},scale=0.25]
	\draw (0,0) -- (0,12);
	\draw (0,12) to [controls=+(45:2) and +(135:2)] (6,12);
	\draw (6,12) -- (6,0);
	\draw (0,0) to [controls=+(45:1) and +(135:1)] (3,0);
	\draw (3,0) to [controls=+(45:1) and +(135:1)] (6,0);
	\end{scope}
	}
    \foreach \xx in {-12,-11.25,...,35.25}{
	\begin{scope}[shift={(\xx,-7.5)},scale=0.125]
	\draw (0,0) -- (0,12);
	\draw (0,12) to [controls=+(45:2) and +(135:2)] (6,12);
	\draw (6,12) -- (6,0);
	\draw (0,0) to [controls=+(45:1) and +(135:1)] (3,0);
	\draw (3,0) to [controls=+(45:1) and +(135:1)] (6,0);
	\end{scope}
	}
	\end{scope}

	\end{tikzpicture}

